QBugs: A Collection of Reproducible Bugs in Quantum Algorithms and a Supporting Infrastructure to Enable Controlled Quantum Software Testing and Debugging Experiments

Reproducibility and comparability of empirical results are at the core tenet of the scientific method in any scientific field. To ease reproducibility of empirical studies, several benchmarks in software engineering research, such as Defects4J, have been developed and widely used. For quantum software engineering research, however, no benchmark has been established yet. In this position paper, we propose a new benchmark -- named QBugs -- which will provide experimental subjects and an experimental infrastructure to ease the evaluation of new research and the reproducibility of previously published results on quantum software engineering.

==> Makefile <==
## Programs
PDFLATEX=pdflatex
BIBTEX=bibtex

TARGET=paper

default: main
main:	$(TARGET).pdf

$(TARGET).pdf: *.tex
	@rm -f $(TARGET).pdf
	$(PDFLATEX) $< $@ || { rm -f *.aux *.idx && false ; }
	$(BIBTEX) $(TARGET) && $(PDFLATEX) $< $@
	if grep -q 'There were undefined references' *.log ; then \
	  $(BIBTEX) $(TARGET) && $(PDFLATEX) $< $@; fi
	while grep -q 'Rerun to get citations correct' *.log ; do \
	  $(PDFLATEX) $< $@ || { rm -f *.aux *.idx && false ; } ; done

# ------------------------------------------------------------------------------
# CLEAN
# ------------------------------------------------------------------------------

clean:
	rm -f *-blx.bib *.aux *.bbl *.blg *.log *.run.xml *.out
	rm -f $(TARGET).pdf

rebuild: clean main

